Identification of Entailment and Contradiction Relations for Natural Language Argumentation: A Neurosymbolic Approach

Argumentation is an important cognitive activity that involves the scrutiny of arguments and counterarguments. When given an argument, it is desirable that its premises entail its claim, and that the premises and claim are consistent, and when given a pair of arguments, it is desirable to check whether one argument supports or attacks another. If the arguments are in natural language, then we could use methods for natural language inference, also known as recognizing textual entailment (RTE). The state-of-the-art RTE methods use machine learning and deep learning, but these are not explainable. An alternative approach which we investigate in this paper is to translate text into an abstract meaning representation (AMR) graph. For this we use a pre-trained AMR parser. We then translate the AMR graph into propositional logic and use a SAT solver for automated reasoning. In text, often common sense suggests that an entailment (or contradiction) relationship holds between a premise and a claim, but because different wordings are used, this is not identified from their logical representations. To address this, we introduce relaxation methods to allow replacement or forgetting of some propositions. Our experimental results show our approach performs well on three RTE datasets. The benefit of our approach is that we have a logical representation of premises and claims, and of the relaxations that are used to identify the entailment and contradiction relations.

==> evaluation.tex <==
\section{Results}

\subsection{Evaluation protocol}
All runs use NumPy's legacy random-number generator with seed 66 and sample
500 examples without replacement from each class, in the order entailment,
neutral, and contradiction. The main experiments and ablations have no sentence-length
limit and use neuro-matching threshold $\tau=0.55$.
For e-SNLI, we use the first 259,999 rows of \texttt{esnli\_train\_1.csv},
retaining rows with string-valued premise, claim, and first explanation.
The no-explanation ablation omits the explanation after this eligibility check,
so the three e-SNLI settings use the same sampled examples.
MultiNLI uses its training partition. SICK pools the cached test, training,
and validation partitions in that order; relation strings are stripped of
surrounding whitespace, and premise--claim direction is selected using the
\texttt{entailment\_AB} relation and class label.
These partition and ordering choices are part of the reported sampling protocol.

We report per-class precision, recall, F1, and support, and overall accuracy.
Support counts the gold examples remaining after excluding \texttt{both} outcomes
and processing errors. A \texttt{both} outcome means that both SAT checks in
Table~\ref{table:classification} return False; it is not assigned to any of the
three labels. Accuracy is the proportion of correct predictions among retained
examples, not among all 1500 sampled examples. We therefore report exclusion counts
alongside the metrics. Because exclusions can change across settings,
comparisons use different retained subsets and are not paired estimates on all
1500 examples. All reported results come from one fixed-seed sample per setting,
not repeated-run estimates.

AMR parsing is batched with batch size 256. Logic is cached by sentence text,
and sentence embeddings are also cached for reuse across settings.
The tables and figures are generated from saved predictions after recomputing
accuracy, class metrics, and confusion matrices. Scores are rounded to three decimals.
\ifdefined\preprintversion
The implementation is available at
\url{https://github.com/fxy-1117/Neurosymbolic-RTE}.
\fi

\begin{table}[t]
\centering
\caption{e-SNLI results on the same 1500 sampled examples.
Accuracy is computed after excluding \texttt{both} outcomes and errors.}
\label{table:esnli}
\small
\setlength{\tabcolsep}{4pt}
\subfloat[Explanations, no forgetting: accuracy \ESNLINoForgetAccuracy{};
\ESNLINoForgetEvaluated{} retained, \ESNLINoForgetBoth{} both, \ESNLINoForgetErrors{} error.
\label{table:esnli:noforget}]{%
\begin{tabular}{lrrrr}
\toprule
Class & Precision & Recall & F1 & Support\\
\midrule
\ESNLINoForgetRows
\bottomrule
\end{tabular}}
\par\medskip
\subfloat[Explanations, forgetting: accuracy \ESNLIMainAccuracy{};
\ESNLIMainEvaluated{} retained, \ESNLIMainBoth{} both, \ESNLIMainErrors{} error.
\label{table:esnli:withforget}]{%
\begin{tabular}{lrrrr}
\toprule
Class & Precision & Recall & F1 & Support\\
\midrule
\ESNLIMainRows
\bottomrule
\end{tabular}}
\par\medskip
\subfloat[No explanations, forgetting: accuracy \ESNLINoExplAccuracy{};
\ESNLINoExplEvaluated{} retained, \ESNLINoExplBoth{} both, \ESNLINoExplErrors{} error.
\label{table:esnli:withoutexplanation}]{%
\begin{tabular}{lrrrr}
\toprule
Class & Precision & Recall & F1 & Support\\
\midrule
\ESNLINoExplRows
\bottomrule
\end{tabular}}
\end{table}

\subsection{Different neuro-matching thresholds}
\label{section:similarity}
For the threshold analysis, we restrict the premise, claim, and explanation
to at most 20 NLTK word tokens each, then sample 500 examples per class with
seed 66. The same 1500 examples are used for all eight thresholds:
$0.50, 0.55, 0.60, 0.65, 0.70, 0.75, 0.80$, and $1.00$.
Explanations and forgetting remain enabled throughout this analysis.
This length-filtered sample differs from the unrestricted main sample.

\begin{figure*}[t]
\centering
\subfloat[Entailment]{\includegraphics[width=.325\textwidth]{threent.pdf}}\hfill
\subfloat[Contradiction]{\includegraphics[width=.325\textwidth]{threcont.pdf}}\hfill
\subfloat[Neutral]{\includegraphics[width=.325\textwidth]{threneu.pdf}}
\caption{Precision, recall, and F1 for the eight neuro-matching thresholds
on the length-filtered e-SNLI sample. Each setting excludes its own \texttt{both}
outcomes; overall accuracy and retained counts are reported in
Table~\ref{table:thresholds}.}
\label{f5}
\end{figure*}

\begin{table}[t]
\centering
\caption{Threshold analysis on 1500 e-SNLI examples with a 20-token limit.
There are no processing errors; retained counts plus \texttt{both} counts equal 1500.}
\label{table:thresholds}
\small
\begin{tabular}{rrrr}
\toprule
$\tau$ & Accuracy & Retained & Both\\
\midrule
\ThresholdRows
\bottomrule
\end{tabular}
\end{table}

As $\tau$ increases from 0.50 to 1.00, entailment precision rises from
0.750 to 0.826, while recall falls from 0.955 to 0.346.
Contradiction recall changes little, from 0.682 to 0.694, while precision
falls from 0.476 to 0.439. Neutral recall increases from 0.030 to 0.099,
but precision falls from 0.179 to 0.100 and F1 remains below 0.100.
Overall accuracy decreases from 0.587 to 0.382.
The highest retained-set accuracy among these eight settings is at $\tau=0.50$;
we retain $\tau=0.55$ for the main experiments rather than select it from this sweep.

At $\tau=1$, forgetting, syntactic matching, and claim simplification are
still enabled. The code accepts neural matches with similarity at least $\tau$,
so this setting is not an ablation of all relaxation methods.
The changing exclusion counts, from 154 at $\tau=0.50$ to 27 at $\tau=1$,
also mean that the curves do not compare identical retained subsets.

\subsection{Pipeline with forgetting versus without forgetting}
Tables~\ref{table:esnli:noforget} and~\ref{table:esnli:withforget}
compare the same unrestricted e-SNLI sample with explanations.
The no-forgetting setting keeps all premise and explanation atoms in the
contradiction check $\phi'\land\psi'$; the forgetting setting instead uses
$\myforget_{\Gamma}(\phi')\land\psi'$. The entailment check and the other
matching and simplification steps are unchanged.

With forgetting, contradiction recall rises from 0.014 to 0.640, but
precision falls from 0.538 to 0.450. Neutral recall falls from 0.716 to
0.023, a decrease of 0.694, and neutral F1 falls from 0.588 to 0.037.
Entailment recall is similar, at 0.928 without forgetting and 0.926 with it.
Retained-set accuracy changes only from \ESNLINoForgetAccuracy{} to
\ESNLIMainAccuracy{}, while the number of \texttt{both} outcomes rises from
\ESNLINoForgetBoth{} to \ESNLIMainBoth{}; each setting also has one processing error.
Thus forgetting increases contradiction recall in this sample, at a substantial
cost to neutral classification and coverage. The small accuracy difference
should not be interpreted as an unqualified improvement.

\subsection{Performance on the three datasets}
\label{section:performance}
For e-SNLI, adding the human explanation to the premise raises retained-set
accuracy from \ESNLINoExplAccuracy{} to \ESNLIMainAccuracy{}.
Entailment recall rises from 0.786 to 0.926 and contradiction recall from
0.030 to 0.640, whereas neutral recall falls from 0.554 to 0.023.
The explanation provides information written to justify the gold relation;
this setting therefore uses more information than ordinary premise--claim NLI.
It is not directly comparable to a system that receives only the two sentences.
The no-explanation setting excludes five \texttt{both} outcomes and one error,
compared with 156 \texttt{both} outcomes and one error when explanations are used.

\begin{table}[t]
\centering
\caption{SICK with forgetting: accuracy \SICKAccuracy{} on \SICKEvaluated{}
retained examples; \SICKBoth{} \texttt{both} outcome and \SICKErrors{} errors.}
\label{table:sick}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrr}
\toprule
Class & Precision & Recall & F1 & Support\\
\midrule
\SICKRows
\bottomrule
\end{tabular}
\end{table}

\begin{table}[t]
\centering
\caption{MultiNLI with forgetting: accuracy \MNLIAccuracy{} on \MNLIEvaluated{}
retained examples; \MNLIBoth{} \texttt{both} outcomes and \MNLIErrors{} error.}
\label{table:mnli}
\small
\setlength{\tabcolsep}{4pt}
\begin{tabular}{lrrrr}
\toprule
Class & Precision & Recall & F1 & Support\\
\midrule
\MNLIRows
\bottomrule
\end{tabular}
\end{table}

SICK has the highest accuracy of the three main settings, at
\SICKAccuracy{}. Its class F1 scores are 0.776 for entailment, 0.855 for
contradiction, and 0.667 for neutral. MultiNLI has accuracy
\MNLIAccuracy{}, with class F1 scores 0.593, 0.446, and 0.531, respectively.
The e-SNLI explanation setting lies between them in overall accuracy, but
has much weaker neutral performance. These results do not establish that
the differences arise solely from common sense requirements, since the
datasets, sampling pools, and available information also differ.

Our pipeline requires no task-specific training in these experiments and
exposes the logical formulas used by the SAT checks. We do not make a
head-to-head accuracy comparison with published learned NLI systems:
their evaluation partitions and input conditions differ from our balanced
samples and explanation-augmented setting.

\section{Discussion}
The pipeline combines pre-trained AMR parsing, propositional translation,
neural matching, and SAT reasoning to identify entailment and contradiction
relations. Its explicit formulas make the final reasoning checks inspectable,
but do not guarantee that the parser or relaxation preserves sentence meaning.
The current results show a strong dependence on dataset and class.
In particular, forgetting improves contradiction recall on the sampled e-SNLI
data while substantially reducing neutral recall and increasing unclassified
\texttt{both} outcomes.

The evaluation is limited to fixed-seed balanced samples rather than complete
official test sets. Reported accuracy excludes conflicting SAT outcomes and
processing errors, so it must be read together with retained counts.
The length-filtered threshold analysis uses a different sample from the main
experiments, and the human explanations in e-SNLI supply label-related information
unavailable in standard two-sentence NLI. Repeated samples and a common held-out
evaluation protocol would be needed to estimate variability and compare directly
with other systems.

For natural language argumentation, future work will test premises and claims
obtained through argument mining~\cite{Lawrence2019}, and investigate how to
combine the pipeline with logic-based approaches to implicit knowledge in
enthymemes~\cite{Hunter2022}. Refining neural matching and controlling which
atoms are forgotten may help reduce the observed confusion between neutral
and contradiction relations.


==> experiment_results.tex <==
% Generated from validated saved predictions; values rounded to three decimals.
\newcommand{\ESNLIMainAccuracy}{0.560}
\newcommand{\ESNLIMainEvaluated}{1343}
\newcommand{\ESNLIMainBoth}{156}
\newcommand{\ESNLIMainErrors}{1}
\newcommand{\ESNLIMainRows}{%
Entailment & 0.734 & 0.926 & 0.819 & 488 \\
Contradiction & 0.450 & 0.640 & 0.529 & 455 \\
Neutral & 0.111 & 0.023 & 0.037 & 400 \\
}
\newcommand{\ESNLINoForgetAccuracy}{0.553}
\newcommand{\ESNLINoForgetEvaluated}{1495}
\newcommand{\ESNLINoForgetBoth}{4}
\newcommand{\ESNLINoForgetErrors}{1}
\newcommand{\ESNLINoForgetRows}{%
Entailment & 0.604 & 0.928 & 0.732 & 500 \\
Contradiction & 0.538 & 0.014 & 0.027 & 498 \\
Neutral & 0.499 & 0.716 & 0.588 & 497 \\
}
\newcommand{\ESNLINoExplAccuracy}{0.456}
\newcommand{\ESNLINoExplEvaluated}{1494}
\newcommand{\ESNLINoExplBoth}{5}
\newcommand{\ESNLINoExplErrors}{1}
\newcommand{\ESNLINoExplRows}{%
Entailment & 0.515 & 0.786 & 0.622 & 495 \\
Contradiction & 0.652 & 0.030 & 0.057 & 499 \\
Neutral & 0.387 & 0.554 & 0.456 & 500 \\
}
\newcommand{\SICKAccuracy}{0.771}
\newcommand{\SICKEvaluated}{1499}
\newcommand{\SICKBoth}{1}
\newcommand{\SICKErrors}{0}
\newcommand{\SICKRows}{%
Entailment & 0.659 & 0.942 & 0.776 & 499 \\
Contradiction & 0.906 & 0.810 & 0.855 & 500 \\
Neutral & 0.826 & 0.560 & 0.667 & 500 \\
}
\newcommand{\MNLIAccuracy}{0.527}
\newcommand{\MNLIEvaluated}{1466}
\newcommand{\MNLIBoth}{33}
\newcommand{\MNLIErrors}{1}
\newcommand{\MNLIRows}{%
Entailment & 0.610 & 0.578 & 0.593 & 476 \\
Contradiction & 0.552 & 0.374 & 0.446 & 494 \\
Neutral & 0.459 & 0.629 & 0.531 & 496 \\
}
\newcommand{\ThresholdRows}{%
0.50 & 0.587 & 1346 & 154 \\
0.55 & 0.584 & 1352 & 148 \\
0.60 & 0.577 & 1356 & 144 \\
0.65 & 0.568 & 1358 & 142 \\
0.70 & 0.550 & 1368 & 132 \\
0.75 & 0.530 & 1384 & 116 \\
0.80 & 0.485 & 1408 & 92 \\
1.00 & 0.382 & 1473 & 27 \\
}

